We're Not Gonna Break It! Consistency-Preserving Operators for Efficient Product Line Configuration

When configuring a software product line, finding a good trade-off between multiple orthogonal quality concerns is a challenging multi-objective optimisation problem. State-of-the-art solutions based on search-based techniques create invalid configurations in intermediate steps, requiring additional repair actions that reduce the efficiency of the search. In this work, we introduce consistency-preserving configuration operators (CPCOs)--genetic operators that maintain valid configurations throughout the entire search. CPCOs bundle coherent sets of changes: the activation or deactivation of a particular feature together with other (de)activations that are needed to preserve validity. In our evaluation, our instantiation of the IBEA algorithm with CPCOs outperforms two state-of-the-art tools for optimal product line configuration in terms of both speed and solution quality. The improvements are especially pronounced in large product lines with thousands of features.

==> ___TODOs.tex <==

Have we resolved the CPCO vs CPCO instance inconsistencies throughout?

Can you help refresh my memory regarding what exactly we wanted to double check in Guo et al?

Alexandru short bio. Jabier added what is written in a previous journal paper of Alexandru, quite short but it might be ok. Also, in the first page it must be "was" with the Department of... but I am not sure.

-------
From the email from Jabier and Steffen response 26/05/2021

Steffen: I will leave these to @Daniel Strüber to look at.
The least element of the parent-child relation is called the "root" feature -> Might be correct, but maybe other way to say it? "The least element" was confusing to me. The common ancestor?
Definition 1, 5) and 6) we should use "exists in c" as in previous ones instead of "is active"
"the naive application of these principles" -> "the naive recursive application of these principles"
Should we say that we tried the naive solution and that is when we identified its limitations? Otherwise they might think we over-engineered things.
"We will present an efficient generation algorithm in Sect. IV." -> "We present our application of these principles through an efficient generation algorithm in Sect. IV."
Theorem 1 and 2: missing ref to the concrete appendix part
"the body set starting from the mandatory features" -> check if you wanted to say core features

Steffen: I haven’t touched this as it is still being rewritten.
"a bit vector, in which each bit represents the activation status of a particular feature" -> to confirm if we use also core features
I am not sure if the CPCO rules previously used (history) can be considered part of the "solution encoding". It is relevant for crossover, but is it really a "solution encoding"? (e.g., not used for fitness calculation)
In CPCO generation we say that our approach does not scale and that we only make 1 instantiation per CPCO and 10 minutes for the generation. "Both of these performance optimizations might affect the completeness of the resulting CPCO suite." -> Completeness here should be again explained, completeness "of the resulting CPCO suite in the sense that not all valid configurations might be reachable".
I don't get the idea of the 10 minutes for the generation. What does it mean? That it might not create CPCOs for the activation or deactivation of some features? How will the approach work without this?
"We study the impact of this decision in our experiments" -> I did not found this in the paper. Maybe is to be added.
"a heuristic "helper" objective (number of deactivated features)." -> it will be nice to add a sentence to provide an intuition about why this is useful

Steffen: I think the comments in the paragraph above are now obsolete after Daniel's fairly comprehensive rewrite of the evaluation sections.

-----
Jabier mentions: I found a couple of sentences like:
"We study the impact of this circumstance as part of our evaluation."
"We study the impact of this decision in our experiments."
Are we really doing that? I mean comparing with and without this decision/circumstance? Or are we just taking the decision and showing the results?

Steffen: Fair point. But we are showing that even with our decisions we are still better than the sota.

Jabier: We probably don't want to conduct new experiments to "study the impact", so I am just saying that these expressions can make it very easy for the reviewers to ask for them.




==> algorithms/cpcos_generationAlgo.tex <==
\begin{algorithm}[tbp]
  \caption{Algorithm for generating CPCOs.}\label{alg:cpcos}
  \begin{algorithmic}[1]
    \footnotesize
    
    \Procedure{generateCPCO}{\textit{feature}, \textit{activate}}
      \LineComment{\textit{feature}: feature to be (de)activated}
      \LineComment{\textit{activate}: activate or deactivate feature?}
      
      \State \textit{rootFeatureInfo} $\gets$ (\textit{feature}, \textit{activate}, true, "")
      \State \textit{candidateActivationChanges} $\gets$ \Call{generateCPCO}{$\emptyset$, \textit{rootFeatureInfo}}\label{alg:cpcos:callRec}
      \State \Call{removeConflicts}{\textit{candidateActivationChanges}}\label{alg:cpcos:filter}
      \State \Return \textit{candidateActivationChanges}
    \EndProcedure
  
  
    \Procedure{generateCPCORec}{\textit{solution}, \textit{featureInfo}} \label{alg:cpcos:startRec}
      \LineComment{\textit{solution}: current partial solution (partial CPCO)}
      \LineComment{\textit{featureInfo}: feature (de)activation to be added to CPCO}

      \If{\textit{featureInfo} $\in$ \textit{solution}}
        \State \Return \textit{solution}
      \EndIf

      \State \textit{solution} $\gets$ \textit{solution} $\cup$ \{\textit{featureInfo}\}

      \If{\textit{activate}}\label{alg:cpcos:startApplyPrinciples}
        \State \textit{extensionCandidates} $\gets$ applyActivationPrinciples(\textit{featureInfo}) 
      \Else
        \State \textit{extensionCandidates} $\gets$ applyDeactivationPrinciples(\textit{featureInfo}) 
      \EndIf\label{alg:cpcos:endApplyPrinciples}
      
      \ForAll{$c \in \textit{extensionCandidates}$}\label{alg:cpcos:startStepDown}
          \State \textit{solution} $\gets$ \Call{generateCPCORec}{\textit{solution}, \textit{c}}
      \EndFor\label{alg:cpcos:endStepDown}

      \State \Return \textit{solution}
    \EndProcedure
  \end{algorithmic}
\end{algorithm}

%
%
%\begin{figure}
%
%\begin{mdframed}
%\footnotesize
%\begin{algorithmic}[1]
%\Procedure{generateCPCO}{\textit{solution}, \textit{feature}, \textit{activate}} 
%\LineComment{\textit{solution}: current partial solution (partial CPCO)}
%\LineComment{\textit{feature}: feature to be (de)activated}
%\LineComment{\textit{activate}: activate or deactivate feature?}
%
%\If{hasIncompatibilities(\textit{\textit{solution}})}
    %\State \textbf{return false}
%\EndIf
%\If{\textbf{not} hasApplicablePrinciples(\textit{solution})}
    %\State \textbf{return true}
%\EndIf
%
%\If{\textit{activate}}
%\State \textit{extensionCandidates} $\gets$ applyActivationPrinciples(\textit{feature}) 
%\Else
%\State \textit{extensionCandidates} $\gets$ applyDeactivationPrinciples(\textit{feature}) 
%\EndIf
%
%
%\ForAll{$c \in \textit{extensionCandidates}$}
    %\State \textit{solution} $\gets$ \textit{solution} $\cup$ \{\textit{c}\} 
    %\State \textit{isComplete} $\gets$ \textsc{generateCPCO}(\textit{solution}, \textit{c}.\textit{feature}, \textit{c}.\textit{activate})
	%\If{\textit{isComplete}}
    %\State \textbf{break}
	%\EndIf
%\EndFor
%\State \textbf{return not} hasIncompatibilities(\textit{solution})
%
%\EndProcedure
%\end{algorithmic}
%
%\smallskip
%
%\noindent{}\textbf{Activation principles.} Let a feature $f$ to be activated be given.
%
%\begin{enumerate}
%%\item \actmand: If $f$ has mandatory children, we activate all mandatory children of $f$.
%\item \actmand:  Activate all mandatory children of $f$.
%\item \actpar: Activate $f$'s parent feature $g$, unless $g$ is a core feature. 
%\item \actreq: If $f$ requires another feature $g$ (via a \textit{requires} relation), activate~$g$.
%\item \actgroup: If $f$ is an "or" or "xor" group,  activate one of $f$'s children.
%\item \actxor: If $f$ is a feature in an "xor" group,  deactivate all of $f$'s siblings.
%\item \actexcl: If $f$ excludes or is excluded by a feature $g$,  deactivate~$g$.
%\end{enumerate}
%
%\smallskip
%
%\noindent{}\textbf{Deactivation principles.} Let a feature $f$ to be deactivated be given.
%
%\begin{enumerate}
%\item \dechild: If $f$ has a non-empty set of active children $G$ (including group members, optional, and mandatory children),  deactivate each child in~$G$.
%%\item \degroup: If $f$ is a "o"' or "xor" group, we activate an inactive child of the group.
%
%\item \dexor: If $f$ is a feature in an "xor" group,  activate one of $f$'s siblings.
%\item \deor: If $f$ is a feature in an "or" group, activate one of $f$'s siblings.
%\item \deparent: If $f$ is a mandatory feature,  deactivate $f$'s parent.
%\item \dereq: If a feature $g$ requires $f$ (via  \textit{requires} relation),  deactivate~$g$.
%\end{enumerate}
%\end{mdframed}
%\caption{Algorithm and principles for generating CPCOs.}\label{alg:cpcos}
%\end{figure}

==> tables/tab_Evaluation_old.tex <==
\begin{table*}[t]
	\caption{\textcolor{red}{(To be updated the entire table)}Comparison of hypervolumes (HV) and execution times (in milliseconds) of the three tools for each feature model. Results show median (MD), and standard deviation (SD) values over 30 runs. Right hand side shows the results of applying the Mann-Whitney U test comparing MDEOptimiser with MODAGAME and SATIBEA, for HV and time, respectively.}
	\label{tab:Evaluation}
	\centering
	\begin{threeparttable}
	%\scriptsize
	\small
	\setlength{\tabcolsep}{2pt}
	\vspace*{-0.4cm}
	\begin{tabular}{l|rrrr|rrrr|rrrr||rr|rr}
		\toprule
		& 
		\multicolumn{4}{c|}{\centering MDEO}
		& \multicolumn{4}{c|}{\centering MODAGAME}
		& \multicolumn{4}{c||}{\centering SATIBEA}
		& \multicolumn{2}{c|}{\centering MDEO HV is greater}
		& \multicolumn{2}{c}{\centering MDEO time is slower}
		\\
		& \multicolumn{2}{c}{\centering HV}
		& \multicolumn{2}{c|}{\centering Time}
		& \multicolumn{2}{c}{\centering HV}
		& \multicolumn{2}{c|}{\centering Time}
		& \multicolumn{2}{c}{\centering HV}
		& \multicolumn{2}{c||}{\centering Time}
		& \multicolumn{1}{c}{\centering MODAGAME}
		& \multicolumn{1}{c|}{\centering SATIBEA}
		& \multicolumn{1}{c}{\centering MODAGAME}
		& \multicolumn{1}{c}{\centering SATIBEA}
		\\
		
		Feature model 
		& \multicolumn{1}{c}{\centering MD} & \multicolumn{1}{c}{\centering SD}
		& \multicolumn{1}{c}{\centering MD} & \multicolumn{1}{c|}{\centering SD}
		
		& \multicolumn{1}{c}{\centering MD} & \multicolumn{1}{c}{\centering SD}
		& \multicolumn{1}{c}{\centering MD} & \multicolumn{1}{c|}{\centering SD}
		
		& \multicolumn{1}{c}{\centering MD} & \multicolumn{1}{c}{\centering SD}
		& \multicolumn{1}{c}{\centering MD} & \multicolumn{1}{c||}{\centering SD}
		
		& \multicolumn{1}{c}{\centering $p$-value} % & $\hat{A}_{12}$
		& \multicolumn{1}{c|}{\centering $p$-value} % & $\hat{A}_{12}$
		
		& \multicolumn{1}{c}{\centering $p$-value} % & $\hat{A}_{12}$
		& \multicolumn{1}{c}{\centering $p$-value} % & $\hat{A}_{12}$
		\\
		
		\midrule
	
	   % {\cellcolor[gray]{.8}}
		x264
		& \hlcell 0.44 &  \hlcell \textbf{0}
		& 2051 & 101

		& 0.43 & 9.85e-6
		& \hlcell 343 & \hlcell 37

		& 0.43 & 1.24e-3
		& 572 & \textbf{30}
		
		& 1.27e-14
		& 5.68-e13
		
		& 1.44e-11
		& 1.43-e11
		\\
		
		BerkeleyDB
		& \hlcell 0.51 & \hlcell \textbf{9.59e-8}
		& 2143 & 146
		
		& 0.51 & 4.92e-3
		& \hlcell 344  & \hlcell 30
		
		& 0.48  & 7.09e-3
		& 599  & \textbf{20}
		
		& 4.05e-13
		& 8.06-e13
		
		& 1.44e-11
		& 1.43-e11
		\\
		
		Wget
		& \hlcell 0.49  & \hlcell 1.43e-3
		& 1965 & 175
		
		& 0.48 & \textbf{2.02e-4}
		& \hlcell 311  & \hlcell \textbf{11}
		
		& 0.45 & 2.25e-3
		& 542  & 15
		
		& 5.18e-12
		& 1.39-e11
		
		& 1.44e-11
		& 1.43-e11
		\\
		
		Sensor Network
		& \hlcell 0.41 & \hlcell 3.78e-3
		& 3048 & 201

		& 0.40 & \textbf{1.77e-3}
		& \hlcell 372  & \hlcell 23
		
		& 0.39 &  4.42e-3
		& 610 &  \textbf{20}
				
		& 6.14e-10
		& 1.44-e11
		
		& 1.44e-11
		& 1.43-e11
		\\
		
		Tank war
		& \hlcell 0.53 & \hlcell \textbf{3.48e-3}
		& 4032  & 237

		& 0.53 &  4.80e-3
		& \hlcell 466 & \hlcell 30
		
		& 0.49 & 9.26-e3
		& 625 &  \textbf{18}
		
		& 0.07
		& 1.44-e11
		
		& 1.44e-11
		& 1.43-e11
		\\
	
		Mobile media
		& \hlcell 0.51 & \hlcell 4.99e-3
		& 3967  & 160

		& 0.50 &  \textbf{1.75e-3}
		& \hlcell 394 & \hlcell \textbf{11}
		
		& 0.44 &  1.16e-2
		& 646 & 20
	
		& 1.75e-11
		& 1.44-e11
		
		& 1.43e-11
		& 1.42-e11
		\\

		WeaFQAs
		& \hlcell 0.37 & \hlcell 3.24e-3
		& 28418 &  825
		
		& 0.15 &  \textbf{3.18e-3}
		& \hlcell 879 &  \hlcell \textbf{36}
		
		& 0.27 & 1.56e-2
		& 1151 & 91
		
		& 1.44e-11
		& 1.44-e11
		
		& 1.44e-11
		& 1.44-e11
		\\
	    
		\bottomrule
	\end{tabular}
\begin{tablenotes}
	\item [] PARAMETERS: (Runs: 30. Population: 100. Evolutions: 50).
%\item [] \colorbox{gray!80}{Highlighted} the best results for hypervolume (HV) and execution time. \textbf{Bold-faced} the most robust results (lowest standard deviation).
\end{tablenotes}
\end{threeparttable}
 \vspace{-0.4cm}
\end{table*}

==> tables/tab_Evaluation_times.tex <==
\begin{table*}[t]
	\caption{Comparison of hypervolumes (HV) for a specific time out (in seconds) of the three tools for each feature model. }
	\label{tab:times}
	\centering
	\begin{threeparttable}
	%\scriptsize
	\footnotesize
	\setlength{\tabcolsep}{2pt}
%	\vspace*{-0.4cm}
	\begin{tabular}{l|r|rr|rr|rr}
		\toprule
		& 
		&
		\multicolumn{2}{c|}{\centering MDEO}
		& \multicolumn{2}{c|}{\centering MODAGAME}
		& \multicolumn{2}{c}{\centering SATIBEA}
		\\

		Feature model 
		& Timeout (s)
		& \multicolumn{1}{c}{\centering Evolutions}
		& \multicolumn{1}{c}{\centering HV} 
		
		& \multicolumn{1}{c}{\centering Evolutions}
		& \multicolumn{1}{c}{\centering HV}
		
		& \multicolumn{1}{c}{\centering Evolutions} 
		& \multicolumn{1}{c}{\centering HV}
		\\
		
		\midrule

		x264
		& 5
		& 5800 &  0.40 % MDEO
		& 38600 & 0.40 % Modagame
		& 25800 & 0.41   % Satibea
		\\

		BerkeleyDB
		& 5
		& 5600 &  0.48 % MDEO
		& 41500 & 0.48 % Modagame
		& 23300 & 0.56   % Satibea
		\\
		
		Wget
		& 5
		& 5500 &  0.45 % MDEO
		& 40700 & 0.45 % Modagame
		& 20900 & 0.42   % Satibea
		\\
		
		Sensor Network
		& 5
		& 4900 &  0.38 % MDEO
		& 35600 & 0.38 % Modagame
		& 23500 & 0.39   % Satibea
		\\
	    
	    Tank war
		& 5
		& 4400 &  0.50 % MDEO
		& 32900 & 0.49 % Modagame
		& 22200 & 0.49   % Satibea
		\\
	
% 		Mobile media
% 		& 5
% 		& 4400 &  0.50 % MDEO
% 		& 32900 & 0.49 % Modagame
% 		& 22200 & 0.49   % Satibea
% 		\\
		
		\bottomrule
	\end{tabular}
\begin{tablenotes}
	%\item [] Runs: 30. Population: 100. Generations: 50 (5000 evolutions).
%\item [] \colorbox{gray!80}{Highlighted} the best results for hypervolume (HV) and execution time. \textbf{Bold-faced} the most robust results (lowest standard deviation).
\end{tablenotes}
\end{threeparttable}
 \vspace{-0.4cm}
\end{table*}

==> tables/tab_FMs_copy.tex <==
\begin{table}[t]
	\caption{Feature models corpus used for evaluation, with number of features, group features (``or'' and ``xor''), core features, cross-tree constraints (CTCs), number of configurations (size of the search space), quality attributes (QAs), and consistency-preserving configuration operators (CPCOs).}
	\label{tab:FMs}
	\centering
	\begin{threeparttable}
	\footnotesize
	\setlength{\tabcolsep}{2pt}
	%\vspace*{-0.4cm}
	\begin{tabular}{lrrrrrr}
		\toprule
		Feature model
% 		& \rotatebox{90}{\small{Features}}
% 		& \rotatebox{90}{\small{Groups}}
% 		& \rotatebox{90}{\small{Core f.}}
% 		& \rotatebox{90}{\small{CTCs}}
% 		& \small{Configs}
% 		& \rotatebox{90}{\small{QAs}}
% 		& \rotatebox{90}{\small{CPCOs}}
	    & \#Features
		& \#Groups
		& \#Core
		& \#CTCs
		& \#Configs
		& \#CPCOs
		\\
		
		\midrule
		Wget~\cite{Siegmund2013}
		& 17
		& 1
		& 2
		& 0
		& 8,192
		& 3
		\\
		
		Tank war~\cite{Siegmund2013} %\tnote{1}
		& 37
		& 8
		& 7
		& 0
		& 580,608
		& 3
		\\
	
		Mobile media~\cite{figueiredo2008evolving}
		& 43
		& 7
		& 10
		& 3
		& 2,128,896
		& 3
		\\

		WeaFQAs~\cite{Horcas2019splc}
		& 179
		& 43
		& 1
		& 7
		& 2.93e24
		& 3
		\\
		
% 		Linux Base~\cite{knuppel2017there}
% 		& 380
% 		& -
% 		& 115
% 		& 0
% 		& -
% 		& 3
% 		\\
		
		Busy Box~\cite{knuppel2017there}
		& 843
		& -
		& 20
		& 33
		& -
		& 3
		\\
		
		EMB ToolKit~\cite{knuppel2017there}
		& 1179
		& -
		& 78
		& 1
		& -
		& 3
		\\
		
		CDL ea2468~\cite{knuppel2017there}
		& 1396
		& -
		& 4
		& 336
		& -
		& 3
		\\
		
		Linux Distribution~\cite{knuppel2017there}
		& 1580
		& -
		& 6
		& 154
		& -
		& 3
		\\
		
	    Linux 2.6.33.3~\cite{knuppel2017there}
		& 6353
		& 137
		& 51
		& 3208
		& -
		& 3
		\\
		
	    Automotive 2.1~\cite{knuppel2017there}
		& 14009
		& 1135
		& 1394
		& 531
		& -
		& 3
		\\
	    
		\bottomrule
	\end{tabular}
%\begin{tablenotes}
    %\item[] \#Features: number of features. \#Groups: group features (``or'' and ``xor''). \#Core: always activated features. \#CTCs: cross-tree constraints. \#Configs: number of configurations (size of the search space). \#QAs: quality attributes. \#CPCOs: Consistency-Preserving Configuration Operators (search operators).
	%\item[1] Developed by L. Lei et al.(U Magdeburg).
	%\item[]
%\end{tablenotes}
\end{threeparttable}
	\vspace*{-0.4cm}
\end{table}
